Data-Driven Feedback Generation for Introductory Programming Exercises

This paper introduces the "Search, Align, and Repair" data-driven program repair framework to automate feedback generation for introductory programming exercises. Distinct from existing techniques, our goal is to develop an efficient, fully automated, and problem-agnostic technique for large or MOOC-scale introductory programming courses. We leverage the large amount of available student submissions in such settings and develop new algorithms for identifying similar programs, aligning correct and incorrect programs, and repairing incorrect programs by finding minimal fixes. We have implemented our technique in the SARFGEN system and evaluated it on thousands of real student attempts from the Microsoft-DEV204.1X edX course and the Microsoft CodeHunt platform. Our results show that SARFGEN can, within two seconds on average, generate concise, useful feedback for 89.7% of the incorrect student submissions. It has been integrated with the Microsoft-DEV204.1X edX class and deployed for production use.

==> formal.tex <==
% note:
% remove language definition which later explanation does 
% not seem to rely on.
% removing most of the equations that are not so necessary.
% the focus is a clear exposition on the terminologies we
% use later

\section{Formalization}
\label{section:formal}

In this section, we give formal definitions to the terminology 
which later expositions relies on. Throughout the section we 
denote $P_{e}$/$P_{c}$ to be an incorrect/correct program.

%In this section, we introduce an imperative programming language \Lan with which 
%we formalize our automated program repair technique.
%
%\begin{figure}[th!]
%	
%	\begin{equation*}
%		\begin{split}
%			\text{Expression}\:\: e :=& \:\: n\:\:|\:\:v\:\:|\:\: (e) \:\:|\:\: e_{0}[e_{1}] \:\:|\:\: e_{0}.e_{1} \:\:|\:\: e_{0} \; op \; e_{1} \:\: |\:\: op \; e \:\:|\:\: \{e_{0},...,e_{n}\} \\
%			& \!\!\! |\:\: e(e_{0},...,e_{n}) \:\:|\:\: e_{0} \: ?\: e_{1} : e_{2} \:\: \\
%			\text{Statement}\:\: s :=& \:\: v := e \:\:|\:\: e_{0}.e_{1} = e \:\:|\:\: e_{0}[e_{1}] = e \:\:|\:\: s_{0}\:;\:s_{1} \:\:|\:\: \mathit{while}(e)\: \mathit{do}\: s \\
%			& \!\!\! |\:\: \mathit{for}(e_{0};e_{1};e_{2})\:\mathit{do}\:s \:\:|\:\: \mathit{foreach}(e_{0}\: in\: e_{1})\:do\:s     \:\:|\:\: \mathit{if}\:e\:\mathit{then}\:s_{0}\:\mathit{else}\:s_{1}  \\
%			& \!\!\! |\:\: \mathit{return}\:s
%		\end{split}
%	\end{equation*}	
%	\caption{The syntax of language \Lan.}
%	\label{fig:lan}
%\end{figure}
%
%\subsection{The Language \Lan}
%The syntax of language \Lan is shown in Figure~\ref{fig:lan}. 
%We describe the features of the language below.
%
%\paragraph{\textbf{Expression}} 
%A constant $n$ is any value from a universal data domain $D$ containing all 
%values in the language such as all integers, characters, Booleans, \etc in 
%\Csharp. $v$ represents a variable. An expression is either a constant $n$, 
%a variable $v$, or some other recursive structures applied to the expression 
%itself such as binary and unary expressions. Here, $op$ represents a 
%set of binary operators such as $+$, $-$, $<$, $||$, $\&$ or a set of 
%unary operators such as $++$, $--$, $!$ and $cast$.
%
%\paragraph{\textbf{Statement}} 
%An imperative program written in Language \Lan may consist of assignment 
%statements to variables, composite data types like class objects or aggregated 
%data type like arrays, lists, maps, \etc; control statements such as 
%branching and looping; and return statement.
%
%\paragraph{\textbf{Semantics}} 
%We assume the standard imperative semantics to execute programs written in \Lan 
%such as the semantics of \Csharp.

%
%\subsection{\textbf{Formal Definitions}}
%In this section, we give the formalization of various terms and concepts used in our program repair technique. 
%We assume a buggy program is denoted by $P_{e}$ and a correct program is denoted by $P_{c}$, where both are written in Language \Lan introduced earlier.
%
%\begin{figure}[th!]
%	
%	\begin{align} 		
%		\mathit{int} \:\: \mathit{max} &= \mathit{Math}.\mathit{Max}(b, 1) \label{exp:f}  \tag{\rom{1}} \\ 
%		\mathit{int} \:\: \mathit{max} &= \mathit{Math}.\mathit{Max}(b, 2) \label{exp:s} \tag{\rom{2}} \\ 
%		\mathit{int} \:\: \mathit{max} &= \mathit{Math}.\mathit{Max}(b, c) \label{exp:t}  \tag{\rom{3}} 
%	\end{align}
%	
%	\caption{Expressions to be modified.}
%	\label{fig:exp}
%\end{figure}
%


\subsection{Syntactic Distance}
If $\mathit{CF}(P_{e}) = \mathit{CF}(P_{c})$
the syntactic distance between $P_{e}$ and 
$P_{c}$, denoted by $\mathcal{D}(P_{e}, P_{c})$, 
will be equal to the \textit{tree edit distance} 
between the AST of $ {P}_{e}$ and $ {P}_{c}$ 
($\Delta({P}_{e},  {P}_{c})$). Here we rely on 
the classical definition of tree edit distance 
which is the minimal-cost sequence of node edit 
operations (\textit{delete/insert/rename}) that 
transforms one tree into another. If 
$\mathit{CF}(P_{e}) \ne \mathit{CF}(P_{c})$, 
we consider $ \mathcal{D}({P}_{e},  {P}_{c})$ 
to be infinity, in other words, syntactically no 
matter how similar to $P_{e}$ $P_{c}$ turns out to 
be it will not be considered in the search procedure. 


\begin{equation}
\mathcal{D}({P}_{e}, {P}_{c}) = 
\begin{cases}
\Delta({P}_{e}, {P}_{c}), & \mathit{CF}({P}_{e}) = \mathit{CF}({P}_{c})  \\
\quad \infty, & \mathit{CF}({P}_{e}) \neq \mathit{CF}({P}_{c})
\end{cases}
\end{equation}


%\paragraph{\textbf{Syntactic Distance}} If 
%%$P_{e}$ and $P_{c}$ 
%%have the identical control flow structure ($\mathit{CFL}(P_{e}) = \mathit{CFL}(P_{c})$), 
%$\mathit{CF}(P_{e}) = \mathit{CF}(P_{c})$
%the syntactic distance between 
%$P_{e}$ and $P_{c}$, denoted by $\mathcal{D}(P_{e}, P_{c})$, 
%will be equal to the \textit{tree edit distance} between the AST of $ {P}_{e}$ 
%and $ {P}_{c}$ ($\Delta({P}_{e},  {P}_{c})$). Here we rely on the classical definition of tree edit 
%distance which is the minimal-cost sequence of node edit operations 
%(\textit{delete/insert/rename}) that transforms 
%one tree into another. 
%%The only change we introduce is to variablize the cost 
%%of operations applied to the leaf nodes. Assuming any operation made to the 
%%intermediate nodes cost one unit, an operation will cost 
%%half of the unit if it is 1) on a leaf node and 2) it did not modify the type of 
%%the leaf node. For example, in 
%%Figure~\ref{fig:exp}, changing Expression~\ref{exp:f} to~\ref{exp:s} will be half the cost of 
%%changing~\ref{exp:f} to~\ref{exp:t}. 
%%since modifying the value of constants does not change the type 
%%of the nodes. 
%If $\mathit{CF}(P_{e}) \ne \mathit{CF}(P_{c})$, 
%%$ {P}_{e}$ and $ {P}_{c}$ do not employ the 
%%same control flow, 
%we consider $ \mathcal{D}({P}_{e},  {P}_{c})$ 
%to be infinity as defined below.
%
%\begin{equation}
%	%\[
%	\mathcal{D}({P}_{e}, {P}_{c}) = 
%	\begin{cases}
%		\Delta({P}_{e}, {P}_{c}), & \mathit{CFL}({P}_{e}) = \mathit{CFL}({P}_{c})  \\
%		\quad \infty, & \mathit{CFL}({P}_{e}) \neq \mathit{CFL}({P}_{c})
%	\end{cases}
%	%\]
%\end{equation}

\begin{figure}[t!]
	\begin{center}
		\includegraphics[width=0.46\textwidth]{figures/pe.pdf}
		\caption{The eight 2-level atomic tree patterns for a 
			label set of $\{a,\epsilon\}$ on the left. 
			Using 2-level characteristic vector to embed 
			the tree on the right: 
			$\langle1,1,0,0,0,0,0,1\rangle$; 
			and 2-level \pavector: 
   		    $\langle \langle4\rangle, \langle3\rangle,....,\langle2\rangle \rangle$.}
		\label{fig:pe}
	\end{center}
\end{figure}

\subsection{Program Embedding}
We briefly describe a new scheme of embedding 
ASTs into numerical vectors and a new distance 
measure to gauge program similarity. Jiang~\etal 
in~\cite{jiang2007deckard} proposed the idea of 
embedding an AST into a characteristic vector 
and convert the program distance based on tree 
edit distance between ASTs to Euclidean distance 
between numerical vectors. 

\paragraph{\textbf{Characteristic Vector}} 
Within a binary tree, an atomic tree pattern is 
parameterized by a parameter $q$, the height of 
the pattern. A $q$-level atomic pattern is a 
complete binary tree of height $q$. Given a 
label set $l$, including the empty label 
$\epsilon$, there are at most $\vert l\vert^{2q-1}$ 
distinct $q$-level atomic patterns. A $q$-level 
characteristic vector of a tree $T$ is 
$\langle b_{1},  ...., b_{n} \rangle$, where $b_{i}$ 
is the number of occurrences of the $i$-th $q$-level 
atomic pattern in $T$. Figure~\ref{fig:pe} depicts 
an example. Given the label set $\{a,\epsilon\}$, 
the tree on the right can be embedded into 
$\langle1,1,0,0,0,0,0,1\rangle$ using 2-level 
characteristic vectors. With ASTs embedding, one can 
use $L_{1}$ norm, \ie \textit{Hamming distance} or 
$L_{2}$ norm, \ie \textit{Euclidean distance} to 
compute their distance. 

\paragraph{\textbf{Position-Aware Characteristic Vector}} 
In order to further enhance the precision of 
the AST embeddings, position-aware characteristic 
vector incorporates more structural information 
into the encoding vectors. In particular, we define 
a $q$-level \pavector to 
%Based on 
%characteristic vector, we propose \textit{Position-Aware Characteristic Vector}. 
%Our goal is to further improve the precision of the AST embeddings.  
%In particular, we explicitly encode the structural information in 
%the embeddings to reduce the gap between characteristic vector and the AST. 
be $\langle \langle b_{1}^{1},....,b_{1}^{n_{1}}\rangle, 
\langle b_{2}^{1},....,b_{2}^{n_{2}} \rangle, 
\langle b_{\vert l \vert^{2q-1} }^{1},....,
b_{\vert l \vert^{2q-1} }^{n_{\vert l\vert^{2q-1}}}\rangle  
\rangle$, where $b_{i}^{j}$ is the height of root node of 
$j$-th $i$-th $q$ level atomic pattern in $T$. Essentially 
we expand each element $b_{i}$ defined in the $q$-level 
characteristic vector into a list of heights for each 
$i$-th $q$-level atomic pattern in 
$T$ ($b_{i} = \vert \langle b_{i}^{1},....,b_{i}^{n_{i}}   
\rangle \vert$). 
Using 2-level \pavector, the same tree in Figure~\ref{fig:pe} 
can be embedded into $\langle \langle4\rangle, \langle3\rangle
,....,\langle2\rangle \rangle$. For brevity, we shorten the $q$-level 
position-aware characteristic vector to be 
$\langle h_{b_{1}},....,h_{b_{\vert l \vert^{2q-1}}} \rangle$ 
where $h_{b_{i}}$ represents the vector of heights of all $i$-th 
$q$-level atomic tree patterns. The distance
%, 
%denoted 
%by $\mathcal{E}d( \langle v_{b_{i}},....,v_{b_{\vert l \vert^{2q-1}}} 
%\rangle, \langle v_{b_{i}}^\prime,....,v_{b_{\vert l \vert^{2q-1}}}^\prime \rangle)$ 
between two $q$-level \pavector is:

\begin{align}
& \sqrt{\sum\limits_{i=1}^{\vert l \vert^{2q-1}} {\vert\vert \mathit{sort}(h_{b_{i}}, \phi) - \mathit{sort}(h_{b_{i}}^\prime, \phi) \vert\vert_{2}^{2} }} \\ 
& \mathit{where} \; \phi = \mathit{max}(\vert h_{b_{i}}\vert, \vert h_{b_{i}}^\prime \vert)
\end{align}

%\begin{align}
%& v_{sb_{i}}, v_{sb_{i}}^\prime  = \mathit{sort}(v_{b_{i}}, v_{b_{i}}^\prime) \label{equ:pe} \\
%& \mathcal{E}d( \langle v_{b_{i}},....,v_{b_{\vert l \vert^{2q-1}}} \rangle, \langle v_{b_{i}}^\prime,....,v_{b_{\vert l \vert^{2q-1}}}^\prime \rangle) = 
%\sqrt{\sum\limits_{i=1}^{\vert l \vert^{2q-1}} {\vert\vert v_{sb_{i}} - v_{sb_{i}}^\prime \vert\vert_{2}^{2} }}
%\end{align}

$\mathit{sort}(h_{b_{i}}, \phi)$ means sorting 
$h_{b_{i}}$ in descending order followed 
by padding zeros to the end if $h_{b_{i}}$ 
happens to be the smaller vector of the two. 
The goal is to normalize $h_{b_{i}}$ 
and $h_{b_{i}}^\prime$ prior to the 
calculation. $\vert\vert ... \vert\vert_{2}^{2}$ 
denotes the square of the L2 norm.






%\paragraph{\textbf{Program Embedding}} 
%We briefly describe a new scheme of embedding ASTs into 
%numerical vectors and a new distance measure to gauge program similarity. 
%Jiang~\etal in~\cite{jiang2007deckard} proposed the idea of embedding an AST into a characteristic vector 
%and convert the program distance based on tree edit distance between ASTs to Euclidean distance 
%between numerical vectors. Within a binary tree, an atomic tree pattern is 
%parameterized by a parameter $q$, the height of the pattern. A $q$-level 
%atomic pattern is a complete binary tree of height $q$. Given a label set 
%$l$, including the empty label $\epsilon$, there are at most 
%$\vert l\vert^{2q-1}$ distinct $q$-level atomic patterns. A 
%$q$-level characteristic vector of a tree $T$ is $\langle b_{1},  ...., b_{n} \rangle$, 
%where $b_{i}$ is the number of occurrences of the $i$-th $q$-level 
%atomic pattern in $T$. Figure~\ref{fig:pe} depicts an example, in which 
%the label set is $\{a,\epsilon\}$. Using 2-level characteristic 
%vectors the tree on the right can be embedded into 
%$\langle1,1,0,0,0,0,0,1\rangle$. With ASTs embedding, one can use 
%$L_{1}$ norm, \ie \textit{Hamming distance} or $L_{2}$ norm, \ie 
%\textit{Euclidean distance} to compute their distance. Based on 
%characteristic vector, we propose \textit{Position-Aware Characteristic Vector}. 
%Our goal is to further improve the precision of the AST embeddings.  
%In particular, we explicitly encode the structural information in 
%the embeddings to reduce the gap between characteristic vector and the AST. 
%We define a $q$-level \pavector to be 
%$\langle \langle b_{1}^{1},....,b_{1}^{n_{1}}\rangle, 
%\langle b_{2}^{1},....,b_{2}^{n_{2}} \rangle, 
%\langle b_{\vert l \vert^{2q-1} }^{1},....,b_{\vert l \vert^{2q-1} }^{n_{\vert l\vert^{2q-1}}}\rangle  \rangle$, 
%where $b_{i}^{j}$ is the height of root node of $j$-th $i$-th $q$ level atomic 
%pattern in $T$. Essentially we expand each element 
%$b_{i}$ defined in the $q$-level characteristic vector into a list 
%of heights for each of the $i$-th $q$-level atomic pattern in $T$
%($b_{i} = \vert \langle b_{i}^{1},....,b_{i}^{n_{i}}   \rangle \vert$). 
%Using 2-level \pavector, the same tree in Figure~\ref{fig:pe} can be embedded into 
%$\langle \langle4\rangle, \langle3\rangle,....,\langle2\rangle \rangle$. 
%We shorten the $q$-level position-aware characteristic vector to be 
%$\langle v_{b_{i}},....,v_{b_{\vert l \vert^{2q-1}}} \rangle$ where 
%$v_{b_{i}}$ represents the vector of heights of $i$-th 
%$q$-level atomic tree pattern. We define the distance, denoted by 
%$\mathcal{E}d( \langle v_{b_{i}},....,v_{b_{\vert l \vert^{2q-1}}} \rangle, \langle v_{b_{i}}^\prime,....,v_{b_{\vert l \vert^{2q-1}}}^\prime \rangle)$ 
%between two $q$-level \pavector to be:
%
%\begin{align}
%	& v_{sb_{i}}, v_{sb_{i}}^\prime  = \mathit{sort}(v_{b_{i}}, v_{b_{i}}^\prime) \label{equ:pe} \\
%	& \mathcal{E}d( \langle v_{b_{i}},....,v_{b_{\vert l \vert^{2q-1}}} \rangle, \langle v_{b_{i}}^\prime,....,v_{b_{\vert l \vert^{2q-1}}}^\prime \rangle) = 
%	\sqrt{\sum\limits_{i=1}^{\vert l \vert^{2q-1}} {\vert\vert v_{sb_{i}} - v_{sb_{i}}^\prime \vert\vert_{2}^{2} }}
%\end{align}
%
%In Equation~\ref{equ:pe}, $sort(v_{b_{i}},v_{b_{i}}^\prime)$ means sorting 
%$v_{b_{i}}$ and $v_{b_{i}}^\prime$ in descending order followed by padding 
%zeros to the end of the smaller vector in order to normalize 
%$v_{b_{i}}$ and $v_{b_{i}}^\prime$ prior to the computation.
%$\vert\vert v_{sb_{i}} - v_{sb_{i}}^\prime \vert\vert_{2}^{2}$ 
%denotes the square of the L2 norm between $v_{sb_{i}}$ and 
%$v_{sb_{i}}^\prime$.

\subsection{Discrepancies}
%\paragraph{\textbf{Discrepancies}} 
%Given ${P}_{e}$ and ${P}_{c}$, 
%$\mathit{CFL}({P}_{e}) = \mathit{CFL}({P}_{c})$, 
Discrepancies, $\mathcal{C}({P}_{e},{P}_{c})$, 
is a list of pairs, $({S}_{e}$,${S}_{c})$, where 
${S}_{e}$/${S}_{c}$ is a non-control statement or 
control predicates in 
${P}_{e}$/${P}_{c}$. The rational is after a 
syntactically similar program is identified it 
must be correctly aligned with the incorrect program 
so the differences between the aligned statements 
can suggest potential corrections. Program alignment 
is an important step to ensure the naturalness and 
minimality of the generated fixes (We defer the 
detailed discussion to Section~\ref{subsection:align}). 
$\mathcal{C}({P}_{e},{P}_{c})$ is the result of the 
program alignment.

%For 
%an accurate matching from ${S}_{e}$ to ${S}_{c}$, we separate 
%${P}_{e}$ and ${P}_{c}$ into a collection of basic 
%blocks, \ie a group of consecutive non-control statements/expressions. We use $\mathcal{B}({P})$ to denote the separation 
%function on program ${P}$ which returns an array of basic blocks, and $\mathcal{B}({P}_{e})[n]$ to denote the basic block at index $n$. 
%Since $\mathit{CFL}({P}_{e}) = \mathit{CFL}({P}_{c})$ we have 
%$\vert \mathcal{B}({P}_{e}) \vert$ = 
%$\vert \mathcal{B}({P}_{c}) \vert$.
%We formally define the discrepancies $\mathcal{C}({P}_{e},{P}_{c})$ in Figure~\ref{fig:disc}.
%
%\begin{figure}[h!]
%	\begin{align}
%		%
%		\mathcal{C}(\mathcal{B}({P}_{e})[n],\mathcal{B}({P}_{c})[n^{\prime}]) = & 
%		\begin{aligned}[t]
%			\Big\{
%			({S}_{e},{S}_{c}) 
%			\mid &
%			{S}_{e} \in \mathcal{B}({P}_{e})[n] \wedge 
%			{S}_{c} \in \mathcal{B}({P}_{c})[n^{\prime}] \; \wedge \\
%			& n \in (0, \vert \mathcal{B}({P}_{e}) \vert) \wedge n^\prime \in (0,\vert \mathcal{B}({P}_{c}) \vert) \wedge n = n^\prime
%			\Big\}
%		\end{aligned} 
%		%
%		\\
%		%
%		\mathcal{C}({P}_{e},{P}_{c}) = &
%		\begin{aligned}[t]
%			\bigcup \limits_{n=0}^{\vert \mathcal{B}({P}_{e})\vert} {\mathcal{C}(\mathcal{B}( {P}_{c})[n],\mathcal{B}( {P}_{e})[n])}
%		\end{aligned}
%		%
%	\end{align}
%	\caption{Formalizing discrepancies $\mathcal{C}( {P}_{e}, {P}_{c})$.}
%	\label{fig:disc}
%\end{figure}
%


\subsection{Fixes}
\label{subsec:fix}


According to $\mathcal{C}({P}_{e},{P}_{c})$, the fixes, 
denoted by $\mathcal{F}({P}_{e},{P}_{c})$ is generated 
as follows:


\begin{itemize}
	\item \textbf{Insertion Fix}: Given a pair $({S}_{e}$,${S}_{c})$, 
	if ${S}_{e} = \emptyset$ meaning ${S}_{c}$ is not aligned to any 
	statement in ${P}_{e}$, an insertion operation will be produced 
	to add ${S}_{c}$.
	
	\item \textbf{Deletion Fix}: Given a pair $({S}_{e}$,${S}_{c})$, 
	if ${S}_{c} = \emptyset$ meaning ${S}_{e}$ is not aligned to any 
	statement in ${P}_{c}$, an deletion operation will be produced 
	to delete ${S}_{e}$.
	
	\item \textbf{Modification Fix}: Given a pair $({S}_{e}$,${S}_{c})$, 
	if ${S}_{c} \ne \emptyset$ and ${S}_{e} \ne \emptyset$, a modification 
	operation will be produced consisting the set of standard tree 
	operations to turn the AST of ${S}_{e}$ to that of ${S}_{c}$.
\end{itemize}




%\paragraph{\textbf{Fixes}} %we uses three kinds of fixes to repair a incorrect program:

%\begin{itemize}
%	\item \textit{modification} operation that consists of a set of standard tree edit operations to modify an statement. 
%	
%	\item \textit{deletion} operation that removes a statement.
%	
%	\item \textit{insertion} operation that adds a new statement. 	
%\end{itemize} 


%        \setcounter{equation}{0}
%\begin{figure}[th!]
%	\begin{numcases}{\begin{aligned}\mathcal{F}(\mathcal{B}( {P}_{e})[n],\\\mathcal{B}( {P}_{c})[n^\prime]) \end{aligned}= }
%		\big\{
%		\mathit{DEL}( {S}_{e}) \mid \forall {S}_{e} \in \mathcal{B}( {P}_{e})[n]
%		\big\}  & $\vert\mathcal{B}( {P}_{c})[n^\prime]\vert = 0$ \label{con:fir}   \label{equ:fc}
%		\\
%		\big\{
%		\mathit{INS}( {S}_{c}) \mid \forall {S}_{c} \in \mathcal{B}( {P}_{c})[n^\prime]
%		\big\} & $\vert\mathcal{B}( {P}_{e})[n]\vert = 0$ \label{con:sec} \label{equ:sc}
%		\\  
%		\big\{
%		\mathit{DEL}( {S}_{e}) 
%		\mid 
%		\forall {S}_{c} \in \mathcal{B}( {P}_{c})[n^\prime] \nexists {S}_{e} \in \mathcal{B}( {P}_{e})[n] & $\vert\mathcal{B}( {P}_{c})[n^\prime]\vert \ne 0 \: \&$  \\
%		\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;
%		(( {S}_{e}, {S}_{c}) \in \mathcal{C}(\mathcal{B}( {P}_{e})[n],\mathcal{B}( {P}_{e})[n^\prime])) \big\} & $\vert\mathcal{B}( {P}_{e})[n]\vert \ne 0$ \label{equ:tc} \notag 
%		\\
%		\big\{
%		\mathit{INS}( {S}_{c}) 
%		\mid 
%		\forall {S}_{e} \in \mathcal{B}( {P}_{e})[n] \nexists {S}_{c} \in \mathcal{B}( {P}_{c})[n^\prime] & $\vert\mathcal{B}( {P}_{c})[n^\prime]\vert \ne 0 \: \&$ \\
%		\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;
%		(( {S}_{e}, {S}_{c}) \in \mathcal{C}(\mathcal{B}( {P}_{e})[n],\mathcal{B}( {P}_{e})[n^\prime])) \big\}& $\vert\mathcal{B}( {P}_{e})[n]\vert \ne 0$ \label{equ:foc} \notag\\
%		\big\{
%		\mathit{MOD}(O) 
%		\mid 
%		\forall O \subset {Q} ({Q} = MOD( {S}_{e}, {S}_{c})            &  $\vert\mathcal{B}( {P}_{c})[n^\prime]\vert \ne 0 \: \&$ \\ 
%		\:\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;	
%		\wedge \mathit{Syntactically\_Correct}(O)) \big\}     &  $\vert\mathcal{B}( {P}_{e})[n]\vert \ne 0$ \label{equ:fic}  	 \notag	 
%	\end{numcases}
%	\begin{equation} \label{equ:aac}
%		\mathcal{F}( {P}_{e},  {P}_{c}) = \bigcup \limits _{n=0}^{\vert \mathcal{B}( {P}_{e})\vert} {\mathcal{F}(\mathcal{B}( {P}_{e})[n], \mathcal{B}( {P}_{c})[n])}
%	\end{equation}
%	\caption{Definition of fixes, $\mathcal{F}( {P}_{e},  {P}_{c})$.}
%	\label{fig:fix}
%\end{figure}
%
%%We formalize those operations to define the fixes in Figure~\ref{fig:fix}. 
%Given discrepancies 
%$\mathcal{C}(\mathcal{B}( {P}_{e})[n],\mathcal{B}( {P}_{e})[n^\prime])$, 
%we produce the fixes (\ie modification, deletion and insertion) based on the following conditions: 
%
%\begin{enumerate}[label*=(\arabic*)] 
%	\item When $\mathcal{B}( {P}_{c})[n^\prime]$ is empty, we define deletion operations, $\mathit{DEL}( {S})$, 
%	removing all statements present in $\mathcal{B}( {P}_{e})[n]$ (Equation~\ref{equ:fc}).
%	\item When $\mathcal{B}( {P}_{e})[n]$ is empty, we define insertion operations, $\mathit{INS}( {S})$, 
%	adding all statements present in $\mathcal{B}( {P}_{c})[n^\prime]$ (Equation~\ref{equ:sc}).
%	\item When neither $\mathcal{B}( {P}_{e})[n]$ nor $\mathcal{B}( {P}_{c})[n^\prime]$ is empty, we define:
%	
%	\begin{enumerate}[label=(\roman*)]
%		\item For statements present in $\mathcal{B}( {P}_{e})[n]$ but not matched to any statement 
%		in $\mathcal{B}( {P}_{c})[n^\prime]$ from 
%		$\mathcal{C}(\mathcal{B}( {P}_{e})[n],\mathcal{B}( {P}_{c})[n^\prime])$, 
%		we define additional deletion operations to remove those statements from $\mathcal{B}( {P}_{e})[n]$ (Equation~\ref{equ:tc}).
%		
%		\item For statements present in $\mathcal{B}( {P}_{c})[n^\prime]$ but not matched to any statement 
%		in $\mathcal{B}( {P}_{e})[n]$ from   
%		$\mathcal{C}(\mathcal{B}( {P}_{e})[n],\mathcal{B}( {P}_{c})[n^\prime])$, 
%		we define additional insertion operations to add those statements into $\mathcal{B}( {P}_{e})[n]$ (Equation~\ref{equ:foc}).
%		
%		\item For a pair of statements ($ {S}_{e} \in \mathcal{B}( {P}_{e})[n]$, $ {S}_{c} \in \mathcal{B}( {P}_{c})[n^\prime]$) 
%		that is recorded in $\mathcal{C}(\mathcal{B}( {P}_{e})[n]$, $\mathcal{B}( {P}_{c})[n^\prime])$, 
%		we define modification operations, 
%		$\mathit{MOD}(O)$, applying all minimal subsets ($O$) of the entire set of tree edit operations, $Q$, to modify 
%		separate parts of a statement in $\mathcal{B}( {P}_{e})[n]$. The intuition is modifying the whole statement may introduce redundancy which we describe next. (Equation~\ref{equ:fic}).
%	\end{enumerate}		
%\end{enumerate}
%
%
%
%Finally, we define the fixes over two programs $ {P}_{e}$ and $ {P}_{c}$ to be 
%the union of fixes collected from all aligned basic blocks (Equation~\ref{equ:aac}).

\paragraph{\textbf{Minimality}} 
$\mathcal{F}({P}_{e},{P}_{c})$ consists of all the 
operations that rewrite $P_{e}$ entirely into $P_{c}$. 
Instead, the minimum set of $\mathcal{F}({P}_{e},{P}_{c})$ 
should be identified, denoted by 
$\mathcal{F}_{m}({P}_{e},{P}_{c})$ which merely fix the 
issues in $P_{c}$ while leaving the correct part unchanged. 
We argue fix minimality is a critical property to hold for 
any program repair technique. Also from the education 
perspective, minimality helps students to pinpoint the exact 
minimal errors in their code, improving their learning efficiency. 
%
%
%
%
%After applying $\mathcal{F}( {P}_{e},  {P}_{c})$, 
%$\tool$ is capable of repairing $ {P}_{e}$ by turning  $ {P}_{e}$ into $ {P}_{c}$. However, 
%many corrections in $\mathcal{F}( {P}_{e},  {P}_{c})$ are unnecessary because
%they are merely syntactic/semantic differences that do not relate to the root cause of the error. As shown in 
%Figure~\ref{fig:subs} and~\ref{fig:sols}, we remove most of the members in $\mathcal{F}( {P}_{e},  {P}_{c})$ to generate 
%the feedback. From the education perspective, this helps students to 
%pinpoint the exact minimal errors in their code.
%%Generating precise feedback would undoubtedly improves iGrader's usability. 
%Equation~\ref{equ:re} defines redundant set of fixes; Equation~\ref{equ:mi1} and~\ref{equ:mi2} define minimum set of fixes, 
%where $\mathit{Apply}(\mathcal{F},  {P})$ 
%is the resulting program after applying $\mathcal{F}$ to $ {P}$.
%
%\begin{figure}[thb!]
%	\begin{align}
%		& \forall \mathcal{F}_{r} \subset \mathcal{F}( {P}_{e},  {P}_{c}) 
%		\; (\mathit{Output}(\mathit{Apply}(\mathcal{F}_{r}, {P}_{e})) = \mathit{Output}( {P}_{e})) \label{equ:re} \\ 
%		%
%		& \exists \mathcal{F}_{m} \subseteq \mathcal{F}( {P}_{e},  {P}_{c}) 
%		\; (\mathit{Output}(\mathit{Apply}(\mathcal{F}_{m}, {P}_{e})) =  \mathit{Output}( {P}_{c})) \label{equ:mi1} \\ 
%		%
%		& \nexists \mathcal{F}_{m}^{\prime} \subset \mathcal{F}_{m} 
%		\; (\mathit{Output}(\mathit{Apply}(\mathcal{F}_{m}, {P}_{e})) = \mathit{Output}(\mathit{Apply}(\mathcal{F}_{m}^{\prime}, {P}_{e}))) \label{equ:mi2}
%		%	& \mathcal{F}_{redu}(\mathcal{P}_{e}, \mathcal{P}_{c})  \subset \mathcal{F}(\mathcal{P}_{err}, \mathcal{P}_{c}) 
%		%	(Apply(\mathcal{F}_{redu}(\mathcal{P}_{err}, \mathcal{P}_{c})) =  \mathcal{P}_{err}^\prime \: \wedge \label{equ:re} \\ 
%		%	& Output(\mathcal{P}_{err}^\prime) = Output(\mathcal{P}_{err}))  \notag \\
%		%	& \nexists \mathcal{F}^\prime(\mathcal{P}_{err}, \mathcal{P}_{cor}) \subset \mathcal{F}_{min}(\mathcal{P}_{err}, \mathcal{P}_{cor})
%		%	(  
%		%	Apply(\mathcal{F}^\prime(\mathcal{P}_{err}, \mathcal{P}_{cor})) = \mathcal{P}_{cor}^\prime \: \wedge \label{equ:mi} \\ 
%		%	& Output(\mathcal{P}_{cor}^\prime) = Output(\mathcal{P}_{cor})
%		%	) \notag
%		%\mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime]) = 
%		%
%		%
%		%
%		%& \mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime]) = 
%		%	\Big\{
%		%	(\mathcal{S}_{err},\mathcal{S}_{cor}) \mid \mathcal{S}_{err} \in \mathcal{B}(\mathcal{P}_{err})[n] \wedge \mathcal{S}_{cor} \in \mathcal{B}(\mathcal{P}_{cor})[n^\prime] \wedge \\ 
%		%&	Modified\_Variable(\mathcal{S}_{err}) \cap Modified\_Variable(\mathcal{S}_{cor}) \neq \emptyset \wedge n = n^\prime		
%		%    \Big\}  \\
%		%& \mathcal{D}(\mathcal{S}_{err}, \mathcal{S}_{cor}) = TED(\mathcal{S}_{err}, \mathcal{S}_{cor})\\
%		%% & \mathcal{D}(\mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{err})[n^\prime])) =
%		%%	\sum \limits_{(\mathcal{S}_{err}, \mathcal{S}_{cor}) \in \mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{err})[n^\prime])}
%		%%    \mathcal{D}(\mathcal{S}_{err}, \mathcal{S}_{cor}) \\	
%		%& \mathcal{D}(\mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime])) = \sum \mathcal{D}(\mathcal{S}_{err}, \mathcal{S}_{cor}) \wedge (\mathcal{S}_{err}, \mathcal{S}_{cor}) \in \\
%		%& \mathcal{C}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime]) \\
%		%& \nexists \mathcal{C}_{i}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime]) \wedge \mathcal{D}(\mathcal{C}_{i}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime])) < \\ 
%		%&  \mathcal{D}(\mathcal{C}_{sel}(\mathcal{B}(\mathcal{P}_{err})[n],\mathcal{B}(\mathcal{P}_{cor})[n^\prime]))
%	\end{align}
%	\caption{Definition of redundancy and minimum set of fixes.}
%	\label{fig:remi}
%\end{figure}
%
%




==> limi.tex <==
\section{Limitations}

%Add multiple program comparison

$\tool$  supports almost all of \Csharp 
language features, and can 
currently provide feedback based on 
minimum fixes on a fairly 
large fraction (89.7\%) 
of student submissions in our benchmark set. 

We now briefly describe some of the limitations 
of $\tool$ . There are two biggest contributing factors to 
$\tool$ 's failure of generating feedback for some benchmarks. First, the problem of control-flow mismatch. About 5\% of total benchmarks fall in this category. Second, some programs require a large amount of fixes exceeding the threshold of 
$\mathcal{F}_{m}({P}_{e}, {P}_{c})$. 
To address the first limitation, a likely 
future avenue is to match program states 
independent of the control-flow structure, \eg 
begin with the matching of execution traces, then 
revert back to the mapping at statements/expressions 
level. Possible solutions to second problem 
is to incorporate state-of-the-art fault localization 
techniques to reduce the overall search space of possible 
fixes; or to group dependent fixes in certain way so 
they can be included/exclude together which will make 
the minimization loop much more efficient.

The scalability could also potentially present a limitation. 
Even though $\tool$ displays a relative stable performance 
when handling larger size programs, the benchmarks 
we consider are coming from introductory programming exercises. 
It is unclear how would $\tool$ respond to more advanced 
problems (\ie at algorithmic level) on HackerRank, 
topcoder, \etc
